Full-Space Approach to Aerodynamic Shape Optimization

Aerodynamic shape optimization (ASO) involves finding an optimal surface while constraining a set of nonlinear partial differential equations (PDE). The conventional approaches use quasi-Newton methods operating in the reduced-space, where the PDE constraints are eliminated at each design step by decoupling the flow solver from the optimizer. Conversely, the full-space Lagrange-Newton-Krylov-Schur (LNKS) approach couples the design and flow iteration by simultaneously minimizing the objective function and improving feasibility of the PDE constraints, which requires less iterations of the forward problem. Additionally, the use of second-order information leads to a number of design iterations independent of the number of control variables. We discuss the necessary ingredients to build an efficient LNKS ASO framework as well as the intricacies of their implementation. The LNKS approach is then compared to reduced-space approaches on a benchmark two-dimensional test case using a high-order discontinuous Galerkin method to discretize the PDE constraint.

==> 9zzz_LUp2invK.tex <==
Perform the equivalent row operation where we add $\Rs^{-1} \Rx$ times the second row to the first row
%\begin{equation}
%\begin{split}
%\begin{bmatrix}
%% Row 1
% \identity_{\state}
% -
% \Rs^{-1} \Rx
% \approxHessian^{-1} \Lyy^T
% + \Rs^{-1} \Rx
% \approxHessian^{-1} \Lyy^T
%&
% \Rs^{-1} \Rx
% \left(
%     \identity_{\des}
%     - \approxHessian^{-1}  \Lzz
% \right)
% -
% \Rs^{-1} \Rx
% \approxHessian^{-1}  \Lyy^T
% \Rs^{-1} \Rx
% + \Rs^{-1} \Rx
% \approxHessian^{-1} 
% \left(
% \Lzz 
% + \Lyy^T \Rs^{-1} \Rx
% \right)
%&
%\bzero
%% Row 2
%\\
% \approxHessian^{-1} \Lyy^T
%&
% \approxHessian^{-1} 
% \left(
% \Lzz 
% + \Lyy^T \Rs^{-1} \Rx
% \right)
%&
%\bzero
%% Row 3
%\\
% \Rs^{-T}  \Lss
%&
% \Rs^{-T} 
% \Lsx
%&
%\identity_{\state}
%\end{bmatrix}
%\end{split}
%,
%\end{equation}

%\begin{equation}
%\begin{split}
%\begin{bmatrix}
%% Row 1
% \identity_{\state}
%&
% \Rs^{-1} \Rx
%&
%\bzero
%% Row 2
%\\
% \approxHessian^{-1} \Lyy^T
%&
% \approxHessian^{-1} 
% \left(
% \Lzz 
% + \Lyy^T \Rs^{-1} \Rx
% \right)
%&
%\bzero
%% Row 3
%\\
% \Rs^{-T}  \Lss
%&
% \Rs^{-T} 
% \Lsx
%&
%\identity_{\state}
%\end{bmatrix}
%\end{split}
%,
%\end{equation}

\begin{equation}
\begin{split}
\mbf{P}_2^{-1} \KKTmat
=
\begin{bmatrix}
\identity_{\state}  &  -\Rs^{-1} \Rx & \bzero \\
\bzero  & \identity_{\des}   & \bzero \\
\bzero  & \bzero & \identity_{\state}
\end{bmatrix}
\begin{bmatrix}
% Row 1
 \identity_{\state}
&
 \Rs^{-1} \Rx
&
\bzero
% Row 2
\\
 \approxHessian^{-1} \Lyy^T
&
 \approxHessian^{-1} 
 \left(
 \Lzz 
 + \Lyy^T \Rs^{-1} \Rx
 \right)
&
\bzero
% Row 3
\\
 \Rs^{-T}  \Lss
&
 \Rs^{-T} 
 \Lsx
&
\identity_{\state}
\end{bmatrix}
\end{split}
,
\label{eq:p2invK_fact}
\end{equation}
Note that the determinant of a matrix product is the product of each matrices' determinant $\det(AB) = \det(A)\det(B)$.
The determinant of the first matrix of \eqref{eq:p2invK_fact} is one, and therefore we are 


==> table/summary_table.tex <==
\def\printnum#1{%
        \expandafter\printnumaux#1\relax
}
\def\printnumaux#1.#2#3\relax{%
        $\ifnum#1>0+\fi#1.#2$%
}
\def\row#1#2{#1&#2&\FPsub\r{#2}{#1}\printnum\r\\}
\begin{table}[ht]
    \centering
\resizebox{\textwidth}{!}
{%
\begin{tabular}{
r % $\ndes$ 
%c % Cycles 
S[table-format=2.0] @{\,\,\( / \)\,}  S[table-format=3.0] @{\,\,\( / \)\,} S[table-format=3.0]
%c % Total Subits. 
S[table-format=4.0] @{\,\,\( / \)\,}  S[table-format=4.0] @{\,\,\( / \)\,} S[table-format=4.0]
%c % Subits./cycle 
S[table-format=4.1] @{\,\,\( / \)\,}  S[table-format=4.1] @{\,\,\( / \)\,} S[table-format=4.1]
%c % Total Work 
S[table-format=6.0] @{\,\,\( / \)\,}  S[table-format=6.0] @{\,\,\( / \)\,} S[table-format=6.0]
%c % Work/cycle
S[table-format=6.0] @{\,\,\( / \)\,}  S[table-format=6.0] @{\,\,\( / \)\,} S[table-format=6.0]
}
\toprule 
\textbf{$\ndes$ }
& \multicolumn{3}{c}{\textbf{Cycles }}
& \multicolumn{3}{c}{\textbf{Total Subits. }}
& \multicolumn{3}{c}{\textbf{Avg. Subits./Cycle }}
& \multicolumn{3}{c}{\textbf{Total Work }}
& \multicolumn{3}{c}{\textbf{Avg. Work/Cycle} } \\
\midrule
\midrule
\multicolumn{16}{c}{\textbf{Full-space $\PFour$}} \\
\midrule                            
20  &  5    & 5    & 5 & 111 & 114 & 110 & 22.2 & 22.8 & 22.0 & 156823 & 191824 & 211612 & 31365 & 38365 & 42322 \\
40  &  5    & 5    & 5 & 162 & 158 & 157 & 32.4 & 31.6 & 31.4 & 223279 & 263734 & 298642 & 44656 & 52747 & 59728 \\
60  &  4    & 5    & 5 & 158 & 194 & 198 & 39.5 & 38.8 & 39.6 & 216478 & 322984 & 368644 & 54120 & 64597 & 73729 \\
80  &  4    & 5    & 5 & 178 & 226 & 227 & 44.5 & 45.2 & 45.4 & 242911 & 372142 & 425227 & 60728 & 74428 & 85045 \\
100 &  4    & 5    & 5 & 199 & 250 & 249 & 49.8 & 50.0 & 49.8 & 271690 & 412345 & 466726 & 67923 & 82469 & 93345 \\
\midrule
\multicolumn{16}{c}{\textbf{ Full-space $\PTwo$}} \\
\midrule                            
20  &  5    & 5    & 5 & 129 & 129 & 130 & 25.8 & 25.8 & 26.0 & 89128  & 106867 & 122558 & 17826 & 21373 & 24512 \\
40  &  4    & 5    & 5 & 146 & 187 & 188 & 36.5 & 37.4 & 37.6 & 100209 & 154178 & 175485 & 25052 & 30836 & 35097 \\
60  &  4    & 5    & 5 & 179 & 220 & 227 & 44.8 & 44.0 & 45.4 & 122730 & 180929 & 211170 & 30683 & 36186 & 42234 \\
80  &  4    & 5    & 5 & 205 & 258 & 265 & 51.2 & 51.6 & 53.0 & 140216 & 212194 & 245468 & 35054 & 42439 & 49094 \\
100 &  4    & 5    & 5 & 228 & 282 & 282 & 57.0 & 56.4 & 56.4 & 155014 & 231328 & 261025 & 38754 & 46266 & 52205 \\
\midrule
\multicolumn{16}{c}{\textbf{ Full-space $\PFourA$}} \\
\midrule                            
20  &  5    & 5    & 5 & 1159 & 1242 & 1322 & 231.8 & 248.4 & 264.4 & 107952 & 116254 & 124526 & 21590 & 23251 & 24905 \\
40  &  5    & 5    & 5 & 1434 & 1567 & 1702 & 286.8 & 313.4 & 340.4 & 133252 & 146154 & 159486 & 26650 & 29231 & 31897 \\
60  &  4    & 5    & 5 & 1308 & 1787 & 1917 & 327.0 & 357.4 & 383.4 & 121480 & 166394 & 179266 & 30370 & 33279 & 35853 \\
80  &  4    & 5    & 5 & 1414 & 1940 & 2080 & 353.5 & 388.0 & 416.0 & 131232 & 180470 & 194259 & 32808 & 36094 & 38852 \\
100 &  4    & 5    & 5 & 1493 & 2051 & 2222 & 373.2 & 410.2 & 444.4 & 138500 & 190682 & 207326 & 34625 & 38136 & 41465 \\
\midrule
\multicolumn{16}{c}{\textbf{ Full-space $\PTwoA$}} \\
\midrule                            
   20  &   5 &    5 &    5 &1198 & 1269 & 1366 &239.6 & 253.8 & 273.2 &  75600 &   80668 &   87594 &  15120 &   16134 &   17519 \\ 
   40  &   5 &    5 &    5 &1487 & 1633 & 1774 &297.4 & 326.6 & 354.8 &  93518 &  103236 &  112890 &  18704 &   20647 &   22578 \\ 
   60  &   4 &    5 &    5 &1351 & 1849 & 1980 &337.8 & 369.8 & 396.0 &  84906 &  116628 &  125662 &  21226 &   23326 &   25132 \\ 
   80  &   4 &    5 &    5 &1461 & 2011 & 2152 &365.2 & 402.2 & 430.4 &  91726 &  126672 &  136323 &  22932 &   25334 &   27265 \\ 
  100  &   4 &    5 &    5 &1555 & 2137 & 2303 &388.8 & 427.4 & 460.6 &  97554 &  134484 &  145688 &  24388 &   26897 &   29138 \\ 
  160  &   4 &    5 &    5 &1726 & 2407 & 2643 &431.5 & 481.4 & 528.6 & 108156 &  151224 &  166768 &  27039 &   30245 &   33354 \\ 
  320  &   5 &    5 &    5 &2646 & 2668 & 2908 &529.2 & 533.6 & 581.6 & 165376 &  167406 &  183195 &  33075 &   33481 &   36639 \\ 
  640  &   5 &    5 &    5 &2920 & 3435 & 3477 &584.0 & 687.0 & 695.4 & 182364 &  214960 &  218476 &  36473 &   42992 &   43695 \\ 
\midrule
\multicolumn{16}{c}{\textbf{Reduced-space Newton}} \\
\midrule
   20  &   4 &    4 &    4 &  67 &   67 &   65 & 16.8 &  16.8 &  16.2 &  53720 &   65945 &   75069 &  13430 &   16486 &   18767 \\ 
   40  &   4 &    4 &    4 &  99 &  103 &  103 & 24.8 &  25.8 &  25.8 &  74450 &   93620 &  108477 &  18612 &   23405 &   27119 \\ 
   60  &   4 &    4 &    4 & 128 &  128 &  129 & 32.0 &  32.0 &  32.2 &  92817 &  113510 &  131148 &  23204 &   28378 &   32787 \\ 
   80  &   4 &    4 &    4 & 143 &  151 &  149 & 35.8 &  37.8 &  37.2 & 102696 &  131540 &  149718 &  25674 &   32885 &   37430 \\ 
  100  &   4 &    4 &    4 & 161 &  164 &  162 & 40.2 &  41.0 &  40.5 & 114141 &  142070 &  161586 &  28535 &   35518 &   40396 \\ 
  160  &   4 &    4 &    4 & 193 &  201 &  206 & 48.2 &  50.2 &  51.5 & 135615 &  171659 &  200328 &  33904 &   42915 &   50082 \\ 
  320  &   4 &    4 &    4 & 249 &  254 &  261 & 62.2 &  63.5 &  65.2 & 173121 &  214331 &  250875 &  43280 &   53583 &   62719 \\ 
  640  &   4 &    4 &    4 & 336 &  359 &  346 & 84.0 &  89.8 &  86.5 & 227757 &  296360 &  326328 &  56939 &   74090 &   81582 \\ 
\midrule
\multicolumn{16}{c}{\textbf{Reduced-space BFGS}} \\
\midrule
20  &  58   & 63   & 67 & \text{--}&\text{--}&\text{--} & \text{--}&\text{--}&\text{--} & 98066  & 150787 & 209150 & 1691 & 2393 & 3122 \\
40  &  75   & 76   & 75 & \text{--}&\text{--}&\text{--} & \text{--}&\text{--}&\text{--} & 128344 & 178091 & 222634 & 1711 & 2343 & 2969 \\
60  &  87   & 92   & 85 & \text{--}&\text{--}&\text{--} & \text{--}&\text{--}&\text{--} & 143917 & 202656 & 242929 & 1654 & 2203 & 2858 \\
80  &  82   & 75   & 87 & \text{--}&\text{--}&\text{--} & \text{--}&\text{--}&\text{--} & 139325 & 183763 & 262457 & 1699 & 2450 & 3017 \\
100 &  91   & 103  & 87 & \text{--}&\text{--}&\text{--} & \text{--}&\text{--}&\text{--} & 151587 & 225152 & 254836 & 1666 & 2186 & 2929 \\
\bottomrule
\end{tabular}
}
    \caption{Convergence summary of the various methods discussed. $x / y / z$ are the data points given for $m = 4000, 9000, 16000$. }
\label{tab:big_table}
\end{table}
%\section{Data}
%\red{TBD if I include this}.
%\begin{table}[]
%    \centering
%\resizebox{\textwidth}{!}
%{%
%\begin{tabular}{ccccccccc}
%\hline 
%$\ndes$ & $\nstate$ & Method & Preconditioner & Cycles & Total Subits. & Subits./cycle & Total Work & Work/cycle \\
%\hline
%\hline
% 20 & 4000 & RS QN & - & 58 & 0 & 0.0 & 98066 & 1690.8 \\
% 40 & 4000 & RS QN & - & 75 & 0 & 0.0 & 128344 & 1711.3 \\
% 60 & 4000 & RS QN & - & 87 & 0 & 0.0 & 143917 & 1654.2 \\
% 80 & 4000 & RS QN & - & 82 & 0 & 0.0 & 139325 & 1699.1 \\
%100 & 4000 & RS QN & - & 91 & 0 & 0.0 & 151587 & 1665.8 \\
% 20 & 9000 & RS QN & - & 63 & 0 & 0.0 & 150787 & 2393.4 \\
% 40 & 9000 & RS QN & - & 76 & 0 & 0.0 & 178091 & 2343.3 \\
% 60 & 9000 & RS QN & - & 92 & 0 & 0.0 & 202656 & 2202.8 \\
% 80 & 9000 & RS QN & - & 75 & 0 & 0.0 & 183763 & 2450.2 \\
%100 & 9000 & RS QN & - & 103 & 0 & 0.0 & 225152 & 2185.9 \\
% 20 & 16000 & RS QN & - & 67 & 0 & 0.0 & 209150 & 3121.6 \\
% 40 & 16000 & RS QN & - & 75 & 0 & 0.0 & 222634 & 2968.5 \\
% 60 & 16000 & RS QN & - & 85 & 0 & 0.0 & 242929 & 2858.0 \\
% 80 & 16000 & RS QN & - & 87 & 0 & 0.0 & 262457 & 3016.7 \\
%100 & 16000 & RS QN & - & 87 & 0 & 0.0 & 254836 & 2929.1 \\
%  20 & 4000 & RS Newton & BFGS & 4 & 67 & 16.8 & 53720 & 13430.0 \\
%  40 & 4000 & RS Newton & BFGS & 4 & 99 & 24.8 & 74450 & 18612.5 \\
%  60 & 4000 & RS Newton & BFGS & 4 & 128 & 32.0 & 92817 & 23204.2 \\
%  80 & 4000 & RS Newton & BFGS & 4 & 143 & 35.8 & 102696 & 25674.0 \\
% 100 & 4000 & RS Newton & BFGS & 4 & 161 & 40.2 & 114141 & 28535.2 \\
%  20 & 9000 & RS Newton & BFGS & 4 & 67 & 16.8 & 65945 & 16486.2 \\
%  40 & 9000 & RS Newton & BFGS & 4 & 103 & 25.8 & 93620 & 23405.0 \\
%  60 & 9000 & RS Newton & BFGS & 4 & 128 & 32.0 & 113510 & 28377.5 \\
%  80 & 9000 & RS Newton & BFGS & 4 & 151 & 37.8 & 131540 & 32885.0 \\
% 100 & 9000 & RS Newton & BFGS & 4 & 164 & 41.0 & 142070 & 35517.5 \\
% 20 & 16000 & RS Newton & BFGS & 4 & 65 & 16.2 & 75069 & 18767.2 \\
% 40 & 16000 & RS Newton & BFGS & 4 & 103 & 25.8 & 108477 & 27119.2 \\
% 60 & 16000 & RS Newton & BFGS & 4 & 129 & 32.2 & 131148 & 32787.0 \\
% 80 & 16000 & RS Newton & BFGS & 4 & 149 & 37.2 & 149718 & 37429.5 \\
%100 & 16000 & RS Newton & BFGS & 4 & 162 & 40.5 & 161586 & 40396.5 \\
%20 & 4000 & FS & $\PFour$ & 5 & 111 & 22.2 & 156823 & 31364.6 \\
%40 & 4000 & FS & $\PFour$ & 5 & 162 & 32.4 & 223279 & 44655.8 \\
%60 & 4000 & FS & $\PFour$ & 4 & 158 & 39.5 & 216478 & 54119.5 \\
%80 & 4000 & FS & $\PFour$ & 4 & 178 & 44.5 & 242911 & 60727.8 \\
%100 & 4000 & FS & $\PFour$ & 4 & 199 & 49.8 & 271690 & 67922.5 \\
%20 & 9000 & FS & $\PFour$ & 5 & 114 & 22.8 & 191824 & 38364.8 \\
%40 & 9000 & FS & $\PFour$ & 5 & 158 & 31.6 & 263734 & 52746.8 \\
%60 & 9000 & FS & $\PFour$ & 5 & 194 & 38.8 & 322984 & 64596.8 \\
%80 & 9000 & FS & $\PFour$ & 5 & 226 & 45.2 & 372142 & 74428.4 \\
%100 & 9000 & FS & $\PFour$ & 5 & 250 & 50.0 & 412345 & 82469.0 \\
%20 & 16000 & FS & $\PFour$ & 5 & 110 & 22.0 & 211612 & 42322.4 \\
%40 & 16000 & FS & $\PFour$ & 5 & 157 & 31.4 & 298642 & 59728.4 \\
%60 & 16000 & FS & $\PFour$ & 5 & 198 & 39.6 & 368644 & 73728.8 \\
%80 & 16000 & FS & $\PFour$ & 5 & 227 & 45.4 & 425227 & 85045.4 \\
%100 & 16000 & FS & $\PFour$ & 5 & 249 & 49.8 & 466726 & 93345.2 \\
%20 & 4000 & FS & $\PTwo$ & 5 & 129 & 25.8 & 89128 & 17825.6 \\
%40 & 4000 & FS & $\PTwo$ & 4 & 146 & 36.5 & 100209 & 25052.2 \\
%60 & 4000 & FS & $\PTwo$ & 4 & 179 & 44.8 & 122730 & 30682.5 \\
%80 & 4000 & FS & $\PTwo$ & 4 & 205 & 51.2 & 140216 & 35054.0 \\
%100 & 4000 & FS & $\PTwo$ & 4 & 228 & 57.0 & 155014 & 38753.5 \\
%20 & 9000 & FS & $\PTwo$ & 5 & 129 & 25.8 & 106867 & 21373.4 \\
%40 & 9000 & FS & $\PTwo$ & 5 & 187 & 37.4 & 154178 & 30835.6 \\
%60 & 9000 & FS & $\PTwo$ & 5 & 220 & 44.0 & 180929 & 36185.8 \\
%80 & 9000 & FS & $\PTwo$ & 5 & 258 & 51.6 & 212194 & 42438.8 \\
%100 & 9000 & FS & $\PTwo$ & 5 & 282 & 56.4 & 231328 & 46265.6 \\
%20 & 16000 & FS & $\PTwo$ & 5 & 130 & 26.0 & 122558 & 24511.6 \\
%40 & 16000 & FS & $\PTwo$ & 5 & 188 & 37.6 & 175485 & 35097.0 \\
%60 & 16000 & FS & $\PTwo$ & 5 & 227 & 45.4 & 211170 & 42234.0 \\
%80 & 16000 & FS & $\PTwo$ & 5 & 265 & 53.0 & 245468 & 49093.6 \\
%100 & 16000 & FS & $\PTwo$ & 5 & 282 & 56.4 & 261025 & 52205.0 \\
%20 & 4000 & FS & $\PFourA$ & 5 & 1159 & 231.8 & 107952 & 21590.4 \\
%40 & 4000 & FS & $\PFourA$ & 5 & 1434 & 286.8 & 133252 & 26650.4 \\
%60 & 4000 & FS & $\PFourA$ & 4 & 1308 & 327.0 & 121480 & 30370.0 \\
%80 & 4000 & FS & $\PFourA$ & 4 & 1414 & 353.5 & 131232 & 32808.0 \\
%100 & 4000 & FS & $\PFourA$ & 4 & 1493 & 373.2 & 138500 & 34625.0 \\
%20 & 9000 & FS & $\PFourA$ & 5 & 1242 & 248.4 & 116254 & 23250.8 \\
%40 & 9000 & FS & $\PFourA$ & 5 & 1567 & 313.4 & 146154 & 29230.8 \\
%60 & 9000 & FS & $\PFourA$ & 5 & 1787 & 357.4 & 166394 & 33278.8 \\
%80 & 9000 & FS & $\PFourA$ & 5 & 1940 & 388.0 & 180470 & 36094.0 \\
%100 & 9000 & FS & $\PFourA$ & 5 & 2051 & 410.2 & 190682 & 38136.4 \\
%20 & 16000 & FS & $\PFourA$ & 5 & 1322 & 264.4 & 124526 & 24905.2 \\
%40 & 16000 & FS & $\PFourA$ & 5 & 1702 & 340.4 & 159486 & 31897.2 \\
%60 & 16000 & FS & $\PFourA$ & 5 & 1917 & 383.4 & 179266 & 35853.2 \\
%80 & 16000 & FS & $\PFourA$ & 5 & 2080 & 416.0 & 194259 & 38851.8 \\
%100 & 16000 & FS & $\PFourA$ & 5 & 2222 & 444.4 & 207326 & 41465.2 \\
%20 & 4000 & FS & $\PTwoA$ & 5 & 1198 & 239.6 & 75600 & 15120.0 \\
%40 & 4000 & FS & $\PTwoA$ & 5 & 1487 & 297.4 & 93518 & 18703.6 \\
%60 & 4000 & FS & $\PTwoA$ & 4 & 1351 & 337.8 & 84906 & 21226.5 \\
%80 & 4000 & FS & $\PTwoA$ & 4 & 1461 & 365.2 & 91726 & 22931.5 \\
%100 & 4000 & FS & $\PTwoA$ & 4 & 1555 & 388.8 & 97554 & 24388.5 \\
%20 & 9000 & FS & $\PTwoA$ & 5 & 1269 & 253.8 & 80668 & 16133.6 \\
%40 & 9000 & FS & $\PTwoA$ & 5 & 1633 & 326.6 & 103236 & 20647.2 \\
%60 & 9000 & FS & $\PTwoA$ & 5 & 1849 & 369.8 & 116628 & 23325.6 \\
%80 & 9000 & FS & $\PTwoA$ & 5 & 2011 & 402.2 & 126672 & 25334.4 \\
%100 & 9000 & FS & $\PTwoA$ & 5 & 2137 & 427.4 & 134484 & 26896.8 \\
%20 & 16000 & FS & $\PTwoA$ & 5 & 1366 & 273.2 & 87594 & 17518.8 \\
%40 & 16000 & FS & $\PTwoA$ & 5 & 1774 & 354.8 & 112890 & 22578.0 \\
%60 & 16000 & FS & $\PTwoA$ & 5 & 1980 & 396.0 & 125662 & 25132.4 \\
%80 & 16000 & FS & $\PTwoA$ & 5 & 2152 & 430.4 & 136323 & 27264.6 \\
%100 & 16000 & FS & $\PTwoA$ & 5 & 2303 & 460.6 & 145688 & 29137.6 \\
%
%\end{tabular}
%}
%\caption{Caption}
%\label{tab:my_label}
%\end{table}
%
%  \begin{table}[]
%      \centering
%  \resizebox{\textwidth}{!}
%  {%
%  \begin{tabular}{
%  r % $\ndes$ 
%  c % $\nstate$ 
%  c % Cycles 
%  c % Total Subits. 
%  c % Subits./cycle 
%  c % Total Work 
%  c % Work/cycle
%  }
%  \toprule 
%  \textbf{$\ndes$ }
%  & \textbf{$\nstate$ }
%  & \textbf{Cycles }
%  & \textbf{Total Subits. }
%  & \textbf{Subits./Cycle }
%  & \textbf{Total Work }
%  & \textbf{Work/Cycle} \\
%  \midrule
%  \midrule
%  \multicolumn{7}{c}{\textbf{Reduced-space BFGS}} \\
%  \midrule
%  20  &  4000 / 9000 / 16000   &   58   / 63   / 67 & - & - & 98066 / 150787 / 209150 & 1690.8 / 2393.4 / 3121.6 \\
%  40  &  4000 / 9000 / 16000   &   75   / 76   / 75 & - & - & 128344 / 178091 / 222634 & 1711.3 2343.3 / 2968.5 \\
%  60  &  4000 / 9000 / 16000   &   87   / 92   / 85 & - & - & 143917 / 202656 / 242929 & 1654.2 / 2202.8 / 2858 \\
%  80  &  4000 / 9000 / 16000   &   82   / 75   / 87 & - & - & 139325 / 183763 / 262457 & 1699.1 / 2450.2 / 3016.7 \\
%  100 &  4000 / 9000 / 16000   &   91   / 103 / 87 & - & - & 151587 / 225152 / 254836 & 1665.8 / 2185.9 / 2929.1 \\
%  \midrule
%  \multicolumn{7}{c}{\textbf{Reduced-space Newton}} \\
%  \midrule
%  20  &  4000 / 9000 / 16000   &   4    / 4    / 4 & 67   / 67   / 65 & 16.8 / 16.8 / 16.2 & 53720 / 65945 / 75069 & 13430 / 16486.2 / 18767.2 \\
%  40  &  4000 / 9000 / 16000   &   4    / 4    / 4 & 99   / 103 / 103 & 24.8 / 25.8 / 25.8 & 74450 / 93620 / 108477 & 18612.5 / 23405 / 27119.2 \\
%  60  &  4000 / 9000 / 16000   &   4    / 4    / 4 & 128 / 128 / 129 & 32   / 32   / 32.2 & 92817 / 113510 / 131148 & 23204.2 / 28377.5 / 32787 \\
%  80  &  4000 / 9000 / 16000   &   4    / 4    / 4 & 143 / 151 / 149 & 35.8 / 37.8 / 37.2 & 102696 / 131540 / 149718 & 25674 / 32885 / 37429.5 \\
%  100 &  4000 / 9000 / 16000   &   4    / 4    / 4 & 161 / 164 / 162 & 40.2 / 41   / 40.5 & 114141 / 142070 / 161586 & 28535.2 / 35517.5 / 40396.5 \\
%  \midrule
%  \multicolumn{7}{c}{\textbf{Full-space $\PFour$}} \\
%  \midrule                            
%  20  &  4000 / 9000 / 16000   &   5    / 5    / 5 & 111 / 114 / 110 & 22.2 / 22.8 / 22 & 156823 / 191824 / 211612 & 31364.6 / 38364.8 / 42322.4 \\
%  40  &  4000 / 9000 / 16000   &   5    / 5    / 5 & 162 / 158 / 157 & 32.4 / 31.6 / 31.4 & 223279 / 263734 / 298642 & 44655.8 / 52746.8 / 59728.4 \\
%  60  &  4000 / 9000 / 16000   &   4    / 5    / 5 & 158 / 194 / 198 & 39.5 / 38.8 / 39.6 & 216478 / 322984 / 368644 & 54119.5 / 64596.8 / 73728.8 \\
%  80  &  4000 / 9000 / 16000   &   4    / 5    / 5 & 178 / 226 / 227 & 44.5 / 45.2 / 45.4 & 242911 / 372142 / 425227 & 60727.8 / 74428.4 / 85045.4 \\
%  100 &  4000 / 9000 / 16000   &   4    / 5    / 5 & 199 / 250 / 249 & 49.8 / 50   / 49.8 & 271690 / 412345 / 466726 & 67922.5 / 82469 / 93345.2 \\
%  \midrule
%  \multicolumn{7}{c}{\textbf{ Full-space $\PTwo$}} \\
%  \midrule                            
%  20  &  4000 / 9000 / 16000   &   5    / 5    / 5 & 129 / 129 / 130 & 25.8 / 25.8 / 26 & 89128 / 106867 / 122558 & 17825.6 / 21373.4 / 24511.6 \\
%  40  &  4000 / 9000 / 16000   &   4    / 5    / 5 & 146 / 187 / 188 & 36.5 / 37.4 / 37.6 & 100209 / 154178 / 175485 & 25052.2 / 30835.6 / 35097 \\
%  60  &  4000 / 9000 / 16000   &   4    / 5    / 5 & 179 / 220 / 227 & 44.8 / 44   / 45.4 & 122730 / 180929 / 211170 & 30682.5 / 36185.8 / 42234 \\
%  80  &  4000 / 9000 / 16000   &   4    / 5    / 5 & 205 / 258 / 265 & 51.2 / 51.6 / 53 & 140216 / 212194 / 245468 & 35054 / 42438.8 / 49093.6 \\
%  100 &  4000 / 9000 / 16000   &   4    / 5    / 5 & 228 / 282 / 282 & 57   / 56.4 / 56.4 & 155014 / 231328 / 261025 & 38753.5 / 46265.6 / 52205 \\
%  \midrule
%  \multicolumn{7}{c}{\textbf{ Full-space $\PFourA$}} \\
%  \midrule                            
%  20  &  4000 / 9000 / 16000   &   5    / 5    / 5 & 1159 / 1242 / 1322 & 231.8 / 248.4 / 264.4 & 107952 / 116254 / 124526 & 21590.4 / 23250.8 / 24905.2 \\
%  40  &  4000 / 9000 / 16000   &   5    / 5    / 5 & 1434 / 1567 / 1702 & 286.8 / 313.4 / 340.4 & 133252 / 146154 / 159486 & 26650.4 / 29230.8 / 31897.2 \\
%  60  &  4000 / 9000 / 16000   &   4    / 5    / 5 & 1308 / 1787 / 1917 & 327 / 357.4 / 383.4 & 121480 / 166394 / 179266 & 30370 / 33278.8 / 35853.2 \\
%  80  &  4000 / 9000 / 16000   &   4    / 5    / 5 & 1414 / 1940 / 2080 & 353.5 / 388 / 416 & 131232 / 180470 / 194259 & 32808 / 36094 / 38851.8 \\
%  100 &  4000 / 9000 / 16000   &   4    / 5    / 5 & 1493 / 2051 / 2222 & 373.2 / 410.2 / 444.4 & 138500 / 190682 / 207326 & 34625 / 38136.4 / 41465.2 \\
%  \midrule
%  \multicolumn{7}{c}{\textbf{ Full-space $\PTwoA$}} \\
%  \midrule                            
%  20  &  4000 / 9000 / 16000   &   5    / 5    / 5 & 1198 / 1269 / 1366 & 239.6 / 253.8 / 273.2 & 75600 / 80668 / 87594 & 15120 / 16133.6 / 17518.8 \\
%  40  &  4000 / 9000 / 16000   &   5    / 5    / 5 & 1487 / 1633 / 1774 & 297.4 / 326.6 / 354.8 & 93518 / 103236 / 112890 & 18703.6 / 20647.2 / 22578 \\
%  60  &  4000 / 9000 / 16000   &   4    / 5    / 5 & 1351 / 1849 / 1980 & 337.8 / 369.8 / 396 & 84906 / 116628 / 125662 & 21226.5 / 23325.6 / 25132.4 \\
%  80  &  4000 / 9000 / 16000   &   4    / 5    / 5 & 1461 / 2011 / 2152 & 365.2 / 402.2 / 430.4 & 91726 / 126672 / 136323 & 22931.5 / 25334.4 / 27264.6 \\
%  100 &  4000 / 9000 / 16000   &   4    / 5    / 5 & 1555 / 2137 / 2303 & 388.8 / 427.4 / 460.6 & 97554 / 134484 / 145688 & 24388.5 / 26896.8 / 29137.6 \\
%  \bottomrule
%  \end{tabular}
%  }
%  \caption{Convergence summary of the various methods discussed. $x / y / z$ are the data points given for $m = 4000, 9000, 16000$.}
%  \label{tab:my_label}
%  \end{table}
